KEEPER: Learning Control-Sufficient Textual Memory for Long-Horizon LLM Agents

Recursive textual memory can carry earlier errors into later updates, yet task performance alone does not establish memory reliability. We define self-consistency bias as the persistence of incorrect claims already present in the incoming memory. We present KEEPER, a comparative analysis of four auxiliary objectives along information-content and update-sensitivity axes within a shared recursive interface, examining how supervision targets relate to agent performance. Among evaluated conditions, reward-related prediction achieve the highest task performance before and after offline reinforcement learning, outperforming joint supervision. A claim-level analysis of one baseline trajectory documents error persistence despite corrective observations. Together, these analyses motivate evaluating error persistence and valid-information retention alongside task outcomes.

==> latex/name.tex <==
\clearpage
\section{Methodology}
\subsection{Overview}
\label{sec:overview}

We consider agents that replace accumulated interaction history with
a recursively generated textual memory.
Following STEP-HRL\~\cite{TODO},
the agent updates the memory from the previous memory, the executed
action, and the resulting observation, conditioned on the current
subtask.
The action policy then uses the updated memory together with the
current subtask and observation.
The memory therefore determines which historical information remains
available for subsequent decisions.
Omitting an irrelevant detail leaves the decision unchanged, whereas
omitting a fact that distinguishes action outcomes can reduce expected
return.
Recursion introduces a further concern: an error in the current memory
becomes part of the input to later updates.

We formulate memory learning as history abstraction for control.
Approximate information state theory connects the adequacy of a
history representation to the preservation of expected rewards and
predictive information about successor states\~\cite{TODO}.
These criteria motivate our research question:
\emph{When recursively generated textual memory replaces interaction
history, which information losses lead to decision loss, and how well
do training objectives and evaluation metrics capture these losses?}
We use decision loss to mean a reduction in expected return caused
by the loss of information needed for action selection.
To investigate this question, we introduce Control-Sufficient Textual
State Abstraction (CSTSA), which specifies four learning objectives
for information preservation and memory updating.
The objectives provide explicit supervision beyond reference-text
likelihood, allowing us to examine how each training signal relates
to generated memory and downstream control.

\paragraph{Reward Preservation.}
Reference-text likelihood supervises the wording and content of a
memory without explicitly identifying which historical distinctions
matter for reward.
We introduce auxiliary reward prediction from the internal
representation used to generate the memory.
The reward targets derive from subtask completion and action-error
signals in logged interactions.
Reward prediction supplies a direct training signal for making
reward-relevant information accessible in the representation.
This design follows the role of reward preservation in information
state theory and latent state learning\~\cite{TODO}.
The resulting objective allows us to examine whether reward
supervision encourages generated memory to retain information useful
for task completion.

\paragraph{Predictive Preservation.}
Histories with similar immediate rewards can still lead to different
future observations and decisions.
Reward supervision alone therefore leaves some future-relevant
distinctions unspecified.
We train a predictor to map the memory-generation representation
to the fixed embedding of the next reference memory and observation.
Predicting this successor context encourages the representation
to retain information that explains how the interaction develops.
The design draws on the predictive requirements of information state
theory and the use of successor prediction in latent state
learning\~\cite{TODO}.
Our objective predicts the observed continuation in logged data,
providing a tractable means of investigating whether predictive
supervision improves the usefulness of textual memory for later
decisions.

\paragraph{Semantic Anchoring.}
Internal representations require an explicit connection to text
before their distances can support a semantic comparison.
We project the memory-generation representation into a fixed sentence
embedding space and align the projection with the reference memory.
A frozen sentence encoder supplies the reference
embeddings\~\cite{TODO}.
Because the encoder remains fixed, optimization cannot change
the reference targets through updates to the encoder.
Semantic Anchoring thus provides a common comparison space for
the projected representations and a semantic baseline against which
to assess reward and predictive supervision.
The alignment targets reference text, while the information retained
in generated memory requires separate evaluation.

\paragraph{Update Stability.}
Information preservation at an individual step leaves open whether
successive updates amplify errors in the incoming memory.
We perturb the previous memory while holding the subtask, executed
action, and observation fixed.
We then penalize changes in the updated representation that exceed
the corresponding change in the incoming text, measured in the fixed
embedding space.
This design draws on the analysis of sensitivity to previous states
in stable recurrent models\~\cite{TODO}.
The penalty discourages local amplification under a fixed
continuation, while Semantic Anchoring connects the compared
representations to reference text.
The resulting objective lets us examine whether reduced sensitivity
during training transfers to more reliable recursive text generation.

CSTSA applies these auxiliary objectives alongside reference-text
likelihood.
Training uses internal representations computed under teacher
forcing, where the model receives reference output tokens.
The objectives therefore implement learning surrogates for the
design principles above.
We distinguish improvements in these surrogates from information
preservation in generated memory and changes in downstream return.
This distinction allows the experiments to assess both the utility
of each learning objective and the extent to which its associated
measure reflects decision loss.

\subsection{Problem Formulation and Design Principles}
\label{sec:problem_design}

\paragraph{Recursive textual memory.}
We consider decision making within a subtask $g$.
At timestep $t$, the local interaction history is
$H_t=(o_0,a_0,\ldots,a_{t-1},o_t)$, where $o_t$ and $a_t$
denote the observation and action, respectively.
Following the textual-state interface of STEP-HRL\~\cite{TODO},
we maintain a memory $p_t$ that summarizes the local history.
For analysis, we fix a deterministic decoding rule and write the
memory update and action selection as
\begin{equation}
\begin{aligned}
p_t &= f_\theta(g,p_{t-1},a_{t-1},o_t), \qquad t\geq 1,\\
z_t &= (g,p_t,o_t), \qquad
a_t \sim \pi^\ell(\cdot\mid z_t),
\end{aligned}
\label{eq:memory_interface}
\end{equation}
where $f_\theta$ is the memory update with parameters $\theta$,
$z_t$ is the decision state, and $\pi^\ell$ is the low-level policy.
We initialize $p_0=\varnothing$ at each subtask boundary.
The recursion induces a history abstraction
$z_t=\alpha_\theta(g,H_t)$.
The memory carries historical information, while the decision state
also provides the current subtask and observation directly.
Our objective is to learn which historical distinctions the memory
retains through successive updates.

\paragraph{Information preservation for control.}
History abstraction becomes problematic when different histories
map to the same decision state despite requiring different
predictions of action consequences.
For example, two histories may yield the same current observation
while differing in whether an earlier prerequisite has been completed.
A memory that omits this distinction can leave the policy unable
to determine the appropriate next action.
Approximate information state theory provides a basis for examining
such abstraction errors through reward and successor prediction,
with decision-quality guarantees under the corresponding
assumptions\~\cite{TODO}.
We adopt these properties as design criteria.
Reward Preservation targets distinctions relevant to immediate
reward, and Predictive Preservation targets distinctions relevant
to subsequent decision states.

\paragraph{Reward preservation.}
An abstract state should retain the information required to predict
the expected reward of an action.
Let $R_{t+1}$ denote the environment reward after action $a$,
and let $\bar r_t(z,a)$ be a reward model defined on abstract states.
For an analysis domain $\mathcal S_t$ of subtask, history, and action
triples $(g,H,a)$, we express approximate reward preservation as
\begin{equation}
\sup_{(g,H,a)\in\mathcal S_t}
\left|
\mathbb E[R_{t+1}\mid g,H,a]
-
\bar r_t\bigl(\alpha_\theta(g,H),a\bigr)
\right|
\leq \varepsilon_{r,t},
\label{eq:reward_preservation_criterion}
\end{equation}
where $\varepsilon_{r,t}\geq 0$ is the allowed reward discrepancy.
The domain $\mathcal S_t$ specifies the histories and actions
covered by the condition.
A small discrepancy means that the abstract state supports reward
prediction across that domain.
This criterion motivates reward supervision as a means of
encouraging the memory-generation representation to retain
reward-relevant information.

\paragraph{Predictive preservation.}
Reward preservation alone leaves distinctions that affect future
decisions unspecified.
Let $Z_{t+1}$ denote the random successor decision state obtained
after the environment transition and memory update.
Let $\bar P_t(\cdot\mid z,a)$ be an abstract successor distribution,
and let $\mathcal V_{t+1}$ be a specified class of bounded real-valued
functions on successor decision states.
We define predictive discrepancy through these functions:
\begin{equation}
\begin{aligned}
\sup_{(g,H,a)\in\mathcal S_t}
\sup_{v\in\mathcal V_{t+1}}
\Bigl|
&\mathbb E[v(Z_{t+1})\mid g,H,a]\\
&-
\mathbb E_{Z'\sim
\bar P_t(\cdot\mid\alpha_\theta(g,H),a)}
[v(Z')]
\Bigr|
\leq \varepsilon_{p,t}.
\end{aligned}
\label{eq:predictive_preservation_criterion}
\end{equation}
Here, $Z'$ is a successor state drawn from the abstract distribution,
$v$ is a comparison function, and $\varepsilon_{p,t}\geq 0$
is the allowed predictive discrepancy.
The inner supremum defines an integral probability metric over
$\mathcal V_{t+1}$.
The choice of this function class determines which differences
between successor distributions the criterion detects.
When the class includes the relevant continuation-value functions,
the criterion controls discrepancies in predicted future value.
This connection motivates successor prediction as supervision for
information that remains useful beyond the immediate reward.

\paragraph{Stability of recursive updates.}
The preceding criteria concern the information available in a
decision state.
Recursive use introduces an additional question: how strongly does
the next memory respond to an error in the previous memory?
Let $\phi$ be a fixed text encoder, and define the embedding distance
$d_\phi(x,y)=\|\phi(x)-\phi(y)\|_2$ for texts $x$ and $y$,
where $\|\cdot\|_2$ denotes the Euclidean norm.
For a fixed update context $u=(g,a,o)$ containing a subtask, executed
action, and resulting observation, we use $f_\theta(p;u)$ as shorthand
for the memory update.
An ideal non-expansion condition is
\begin{equation}
d_\phi\bigl(f_\theta(p;u),f_\theta(\widetilde p;u)\bigr)
\leq L_f\,d_\phi(p,\widetilde p),
\qquad L_f\leq 1,
\label{eq:update_stability_criterion}
\end{equation}
where $\widetilde p$ is an alternative incoming memory and $L_f$
is an expansion bound over the memory pairs and contexts under
consideration.
Under an identical sequence of update contexts, this condition
prevents the initial embedding discrepancy from growing through
the updates.
The condition motivates sensitivity regularization, following the
stability perspective on recurrent models\~\cite{TODO}.
Its scope is local memory updating: information recovery and
closed-loop trajectories with different actions require separate
analysis.

\paragraph{From design criteria to learning objectives.}
The ideal criteria specify properties of history abstraction,
whereas offline data provide realized actions and outcomes.
We therefore construct learning surrogates from the available
reward-related signals and successor contexts.
Reward Preservation and Predictive Preservation supervise the
internal representation used for memory generation.
Semantic Anchoring aligns a projected representation with fixed
reference-text embeddings, providing a common space for comparing
representations.
Update Stability penalizes excessive sensitivity to perturbations
of incoming memory in that space.
These objectives operate on representations computed under teacher
forcing, so their optimization and the properties of decoded memory
remain distinct.
The following sections define the differentiable interface and
objectives; evaluation examines whether their effects transfer to
information preservation in generated memory and downstream return.

\subsection{Differentiable Memory Representation}
\label{sec:differentiable_memory}

The criteria in Section\~\ref{sec:problem_design} describe which
information textual memory should preserve and how memory updates
should respond to perturbations.
Applying auxiliary supervision through decoded text is difficult
because discrete token selection interrupts ordinary
backpropagation.
We therefore use the memory generator's internal representation
as a differentiable training interface.
Auxiliary objectives computed from this representation provide
gradients to parameters used for memory generation.

\paragraph{Reference-conditioned representation.}
Let $\mathcal D$ denote an offline dataset of logged interactions
with reference memories.
The superscript $\star$ distinguishes reference text from memory
generated by the current model.
For the update at timestep $t$, we construct the reference context
\begin{equation}
x_t^\star =
\bigl(g,p_{t-1}^\star,a_{t-1},o_t\bigr),
\label{eq:reference_memory_context}
\end{equation}
where $g$ is the current subtask, $p_{t-1}^\star$ is the previous
reference memory, $a_{t-1}$ is the executed action, and $o_t$ is
the resulting observation.
We serialize the context using labeled fields and append the
reference output $p_t^\star$.
The field labels specify the input structure, while the output
is a natural-language memory string.

During training, teacher forcing supplies the reference output
tokens to the generator.
We extract $h_t\in\mathbb R^{d_{\mathrm{model}}}$ from the final
transformer layer at the end-of-sequence token appended to
$p_t^\star$, where $d_{\mathrm{model}}$ is the hidden dimension.
This position has causal access to the update context and the
complete reference output.
The resulting representation allows auxiliary predictors to
read information available during the memory update.

\paragraph{Text embedding space.}
To compare internal representations with textual changes,
we introduce a fixed text embedding space.
A frozen Sentence-BERT encoder\~\cite{TODO}
$\phi:\mathcal T\rightarrow\mathbb R^d$ maps a text string
from the space $\mathcal T$ to a unit-normalized vector,
where $d$ is the embedding dimension.
We use the embedding distance defined in
Section\~\ref{sec:problem_design}:
\begin{equation}
d_\phi(x,y)=\|\phi(x)-\phi(y)\|_2,
\qquad x,y\in\mathcal T,
\label{eq:fixed_text_distance}
\end{equation}
where $\|\cdot\|_2$ denotes the Euclidean norm.
The same encoder and preprocessing produce reference-memory
targets, successor-context targets, and incoming-memory
perturbation distances during training.
Freezing the encoder prevents parameter updates from changing
these targets and input distances through the encoder.

\paragraph{Projected memory representation.}
The generator's hidden representation and the text embeddings
occupy different spaces.
We introduce a learned projection
$\psi_\theta:\mathbb R^{d_{\mathrm{model}}}\rightarrow\mathbb R^d$
and normalize its output:
\begin{equation}
q_t=
\frac{\psi_\theta(h_t)}
{\|\psi_\theta(h_t)\|_2},
\label{eq:projected_memory_representation}
\end{equation}
for nonzero projection outputs.
Here, $q_t$ is the projected memory representation, and $\theta$
includes the projection parameters alongside the generator's
trainable adapter parameters.
Semantic Anchoring supervises $q_t$ with the reference embedding
$\phi(p_t^\star)$.
The alignment gives the projected representation an explicit
reference target in the text embedding space.

Update Stability uses this projection to compare representations
obtained from original and perturbed incoming memories.
Reward Preservation and Predictive Preservation instead read
$h_t$ directly.
The predictors therefore use the contextual hidden representation,
while the stability objective uses a representation trained
against reference-text embeddings.
The next section defines the corresponding objectives and their
gradient paths.

\paragraph{Training representations and generated memory.}
The vector $q_t$ depends on both the update context and the
teacher-forced reference output.
Consequently, information accessible in $q_t$ can differ from
information expressed in an independently generated memory.
The pretrained backbone weights remain frozen, and auxiliary
gradients update the trainable adapter and heads according to
the optimization rules specified below.
At inference, the generator produces textual memory recursively,
and the action policy consumes that text with the subtask and
current observation.
The projection and auxiliary predictors support training;
the action policy receives the generated memory rather than
$q_t$.
We therefore evaluate generated-text information preservation
separately from auxiliary prediction accuracy.

\subsection{Optimization and Deployment}
\label{sec:optimization_deployment}

Auxiliary prediction and sensitivity objectives supervise internal
representations, while memory generation also requires direct
supervision of the output text.
We therefore train the generator with reference-text likelihood
alongside the four auxiliary objectives:
\begin{equation}
\begin{aligned}
\mathcal L_{\mathrm{CSTSA}}
={}& \mathcal L_{\mathrm{BC}}
+\lambda_a\mathcal L_{\mathrm{align}}
+\lambda_r\mathcal L_{\mathrm{reward}}\\
&+\lambda_p\mathcal L_{\mathrm{selfpred}}
+\lambda_f\mathcal L_{\mathrm{nonexp}}.
\end{aligned}
\label{eq:cstsa_training_objective}
\end{equation}
Here, $\mathcal L_{\mathrm{BC}}$ is the behavioral cloning
objective.
The auxiliary terms correspond to Semantic Anchoring,
Reward Preservation, Predictive Preservation, and Update Stability,
respectively.
The nonnegative coefficients $\lambda_a$, $\lambda_r$,
$\lambda_p$, and $\lambda_f$ control their contributions.
Reference likelihood supervises the textual output, while the
auxiliary objectives provide additional signals for the information
accessible during memory generation.

\paragraph{Reference supervision.}
For memory generation, behavioral cloning uses the reference
context $x_t^\star$ and reference output $p_t^\star$ defined in
Section\~\ref{sec:differentiable_memory}.
We compute negative log-likelihood averaged over output tokens,
including the appended end-of-sequence token, and then average
over examples.
Both the incoming memory and output supervision use reference
text.
This objective directly supervises which content the generator
expresses and how the generator realizes that content as text.
The aggregated term $\mathcal L_{\mathrm{BC}}$ also includes
the high-level and low-level policy losses whenever their
scheduled updates are active.

\paragraph{Auxiliary gradient paths.}
We compute auxiliary objectives under teacher forcing, without
sampling memory text inside the training loop.
Predictive Preservation uses examples with an available successor
target, and Update Stability uses examples with a valid
incoming-memory perturbation.
For Update Stability, we stop gradients through the representationㄴㄴ
from the original input and propagate gradients through the
perturbed branch.
The original representation therefore provides a fixed target
within each paired comparison, while the perturbed branch receives
the sensitivity penalty.

Reward Preservation uses a warmup period to separate initial
reward-head fitting from representation learning.
During warmup, the reward head reads a detached memory-generation
representation, so the reward loss updates the head alone.
After warmup, the same loss also updates the trainable generator
parameters.
This schedule prevents the initially untrained reward head from
directly changing the generator through the reward objective.

When reward supervision is active, we additionally fit the shared
reward head on logged low-level action outputs.
The head reads the detached hidden representation at the end of
each action output and predicts the corresponding auxiliary
reward target.
We weight this measurement loss by $\lambda_r$.
This additional fitting updates the reward head without sending
a direct gradient to the generator through the action
representation.
The fitted head remains shared with the memory-side reward
objective.

\paragraph{Trainable parameters.}
The pretrained backbone and sentence encoder remain frozen.
We train low-rank adaptation (LoRA) parameters\~\cite{TODO}
and the auxiliary projection and prediction heads.
In the shared-adapter configuration, the high-level policy,
low-level policy, and memory generator use the same trainable
adapter.
Behavioral cloning updates the adapter through each active policy
loss, and auxiliary objectives update the adapter through the
memory-generation representation.
Parameter sharing therefore allows memory objectives to affect
action selection through both generated text and changes to the
shared policy parameters.
We interpret downstream results from this configuration as
effects on the jointly trained agent.

\paragraph{Recursive deployment.}
At the beginning of a subtask, the high-level policy supplies
the natural-language goal, and the agent initializes the local
memory to an empty state.
The low-level policy selects an action from the subtask,
current observation, and current memory.
After execution, the environment returns a new observation.
The memory generator then uses the previous memory, executed
action, and resulting observation to produce the next memory
under the fixed decoding rule.
The agent repeats this process while the subtask continues.
The sentence encoder, projection, auxiliary predictors, and
perturbation procedure are absent from this action-selection
path.

The optimization above defines the supervised memory-learning
stage.
Any subsequent reinforcement learning stage introduces a separate
policy optimization procedure.
Its interpretation depends on the initialization checkpoint,
training data, critic configuration, and whether auxiliary
objectives remain active.
Accordingly, the supervised objectives and subsequent
reinforcement learning procedure require separate specifications.
